Continual Prototype Evolution: Learning Online from Non-Stationary Data Streams

Attaining prototypical features to represent class distributions is well established in representation learning. However, learning prototypes online from streaming data proves a challenging endeavor as they rapidly become outdated, caused by an ever-changing parameter space during the learning process. Additionally, continual learning does not assume the data stream to be stationary, typically resulting in catastrophic forgetting of previous knowledge. As a first, we introduce a system addressing both problems, where prototypes evolve continually in a shared latent space, enabling learning and prediction at any point in time. In contrast to the major body of work in continual learning, data streams are processed in an online fashion, without additional task-information, and an efficient memory scheme provides robustness to imbalanced data streams. Besides nearest neighbor based prediction, learning is facilitated by a novel objective function, encouraging cluster density about the class prototype and increased inter-class variance. Furthermore, the latent space quality is elevated by pseudo-prototypes in each batch, constituted by replay of exemplars from memory. As an additional contribution, we generalize the existing paradigms in continual learning to incorporate data incremental learning from data streams by formalizing a two-agent learner-evaluator framework. We obtain state-of-the-art performance by a significant margin on eight benchmarks, including three highly imbalanced data streams.

==> apdx.tex <==
\section*{Appendix}


\section{Algorithm}
\label{apdx:algor}
Our proposed algorithm is fully formalized in this section, as well as in our code that will be made publicly available on acceptance of this paper.
Algorithm~\ref{main_algor} and Algorithm~\ref{sub_algor} describe the learner for CoPE, whereas the evaluator uses $c^* = \argmax_{c \in \mathcal{Y}} {\bf f}_i^T \  {\bf p}^c$, classifying ${\bf x}_i$ as category $c^*$ with the most similar prototype ${\bf p}^{c^*}$.
As for a true continually progressing system, the evaluator can urge prediction at any point in time, while the learner keeps acquiring knowledge from the data stream.

  \renewcommand{\algorithmicensure}{\textbf{Initialize }}
  \newcommand{\mattalgorcomment}[1]{\Statex\textit{// #1}}
\algdef{SE}[DOWHILE]{Do}{doWhile}{\algorithmicdo}[1]{\algorithmicwhile\ #1}%

\begin{minipage}{1\textwidth}
\begin{algorithm}[H]

\begin{algorithmic}[1] %

\Require data stream $S$, prototype momentum $\alpha$, memory capacity $M$, learning rate $\eta$
\Ensure operational memory $\mathcal{M}=\emptyset$, observed classes $\mathcal{Y}=\emptyset$, sample count per class $N=\emptyset$, model parameters~${\bf \theta}$
\For {$B_n=\{({\bf x}_1, {\bf y}_1), ... , ({\bf x}_{|B_n|}, {\bf y}_{{|B_n|}}) \}  \sim S$}  \Comment{Data stream batch w/o task information}
\State $B_{\mathcal{M}} \leftarrow \textsc{RandomSample}(\mathcal{M}_r, |B_n|)$ \Comment{Randomly sample $|B_n|$ exemplars from $\mathcal{M}_r$}
\State $\mathcal{B} = \emptyset$
\For {$({\bf x}_i, {\bf y}_i) \in B_n \cup B_{\mathcal{M}}$}

\If {$y_i \notin \mathcal{Y}$}
\State \textsc{InitClass}$(\mathcal{M}, N, \mathcal{Y}, y_i)$ \Comment{Initialize memory and prototype}
\EndIf
\State $\mathcal{B} \leftarrow \mathcal{B} \cup f_{\theta}({\bf x}_i)$ \Comment{Collect features}
\EndFor

\State $\mathcal{L} \leftarrow 0$ \Comment{Initialize loss}

\For {${\bf f}_i^c \in \mathcal{B}$}
\State $\mathcal{L} \leftarrow \mathcal{L}  - \frac{1}{|\mathcal{B}|} \left[ \log P(c |{\bf x}_i^c) + \sum_{{\bf x}_j^k} \log(1- P(c|{\bf x}_j^k)) \right]$ \Comment{Sum al instances PPP-loss}
\EndFor

\State ${\bf \theta} \leftarrow {\bf \theta} + \eta \ \nabla \mathcal{L} $ \Comment{Optimize objective with SGD}

\State \textsc{PrototypeUpdate}$(\mathcal{M}_p, \mathcal{B}, N, \alpha)$ \Comment{Update prototypes in $\mathcal{M}_p$}
\State \textsc{MemoryUpdate}$(\mathcal{M}_r, B_n, N)$ \Comment{Update memory $\mathcal{M}_r$ with new input samples}

\EndFor
\end{algorithmic}
\caption{\label{main_algor} The CoPE learner in the data incremental learning setup. }
\label{algor:framework}
\end{algorithm}
\end{minipage}


\begin{algorithm*}[H]

\begin{minipage}[t]{0.5\linewidth}
\begin{algorithmic}[1] %
\Require memory capacity $M$
\Function{InitClass}{$\mathcal{M}, N, \mathcal{Y}, y$}
\State $N \leftarrow N \cup \{N^y=0\}$ \Comment{Sample counts}
\State $\mathcal{Y} \leftarrow \mathcal{Y} \cup \{y\}$ \Comment{Observed classes}
\State $m = M / |\mathcal{Y}|$ \Comment{Capacity per class}
\For{$\mathcal{M}^c_r= ({\bf x}_1,...,{\bf x}_{|\mathcal{M}^c_r|}) \in \mathcal{M}_r$}
\State $\mathcal{M}^c_r \leftarrow ({\bf x}_1,...,{\bf x}_m)$ \Comment{Keep first $m$}
\EndFor
\State $\mathcal{M} \leftarrow \mathcal{M} \cup \{\mathcal{M}^y = \emptyset \}$ %
\State ${\bf p}^y \leftarrow \textsc{Uniform}^d(0,1)$
\State $\mathcal{M}_p^y \leftarrow \{{\bf p}^y / ||{\bf p}^y||_2\}$ \Comment{Init prototype}
\EndFunction

\end{algorithmic}
\end{minipage}
\hfill
\begin{minipage}[t]{0.5\linewidth}
\begin{algorithmic}[1] %
\Function{PrototypeUpdate}{$\mathcal{M}_p, \mathcal{B}, N, \alpha$}
\For {${\bf  p}^c \in \mathcal{M}_p$}
    \State $N^c \leftarrow N^c + |\mathcal{B}^c|$
    \State ${\bf \Bar{p}}^c = \frac{1}{|\mathcal{B}^c|} \sum_{{\bf f}^c \in \mathcal{B}^c}{\bf f}^c$
    \State ${\bf  p}^c \leftarrow \alpha {\bf  p^c} + (1 - \alpha) {\bf \Bar{p}^c}$
    \State ${\bf  p}^c \leftarrow {\bf  p}^c / ||{\bf  p}^c||_2$
    \Comment{Normalize}
\EndFor
\EndFunction

\Function{MemoryUpdate}{$\mathcal{M}_r, B_n, N$}
\For {${\bf x}_i^c \in B_n$} \Comment{Class Reservoir}
\State $j = \textsc{Uniform}^{\mathbb{N}^1}(1,N^c)$
\If{$ j \leq |\mathcal{M}^c_r|$}
\State $\mathcal{M}^c_r\, [j] \leftarrow {\bf x}_i^c$ \Comment{Replace exemplar}
\EndIf
\EndFor
\EndFunction
\end{algorithmic}
\end{minipage}

\caption{\label{sub_algor} Memory Management of the replay memory and prototypes. $\textsc{Uniform}^{\mathbb{R}^d}(s_1,s_2)$ samples elements in a $d$-dimensional vector with uniform probability in range $[s_1,s_2] \in \mathbb{R}$. 
}
\label{algor:framework_memmanagement}
\end{algorithm*}












\section{Setup}
\label{apdx:setup}
A gridsearch in the online continual learning setup was adopted, selecting the setup with highest performance, similar to \cite{lopez2017gradient}. All methods are prone to learning rate gridsearch $[ 0.05, 0.01, 0.005, 0.001]$. 
iCaRL knowledge distillation strength is set to $1$, and GEM bias is set to $0.5$, following \cite{lopez2017gradient, rebuffi2017icarl,aljundi2019gradient}.
GSS and MIR follow their original setup from their codebase in \cite{aljundi2019gradient} and \cite{aljundi2019online}, with our additional learning rate gridsearch.
CURL~\cite{rao2019continual} and DN-CPM~\cite{lee2020neural} results, and the best imbalanced Split-MNIST results out of the greedy/IQP versions for GSS~\cite{aljundi2019gradient} are reported from their original works. CoPE searched for a suitable temperature $\tau=[0.1,0.2,...,1,2]$ which was set to $0.1$ for all balanced and imbalanced Split-MNIST and Split-CIFAR10 experiments, similar to \cite{ye2019unsupervised}.
Based on the ablation study in Appendix~\ref{apdx:ablation}, we set the prototypical momentum fixed to $0.99$.
For the challenging Split-CIFAR100 setting methods are allowed multiple iterations per batch as in \cite{lopez2017gradient}, from which the best results are selected (baselines, reservoir, CN-DPM perform 1 iteration, others 5). The CIFAR100 temperature required higher concentration with $\tau=0.05$ and prototypical momentum~$0.9$.
For the balanced setups, the latent dimensionality $d$ is fixed to $100$ for Split-MNIST as in~\cite{rao2019continual}, and selected $256$ in a gridsearch $[128, 256]$ and  $[128, 256,512]$ for Split-CIFAR10 and Split-CIFAR100 respectively. 
The imbalanced benchmarks follow the low capacity setup in Appendix~\ref{apdx:extra_exps:lowcap}, with $d \in [16,32,64]$ set to $64$ for Split-MNIST and  $d \in [128, 256]$ set to $128$ for Split-CIFAR10 and $256$ for Split-CIFAR100, with $|\mathcal{M}_r|$ set to $0.3$k, $1$k and $5$k respectively.
Results are obtained without L2 normalization of the prototypes as we found it to have insignificant effect.
The CIFAR10 labels in the confusion matrices from 0 to 10 stand for the indices in the following list:  [\emph{airplane, automobile, bird, cat, deer, dog, frog, horse, ship, truck}].
We will make our code publicly available upon acceptance of this paper to ensure reproducibility.


\section{Resource analysis task-free replay methods}
\label{apdx:res_analysis}
In this section we compare usage of computational and memory resources for the replay methods fitted for the online data incremental learning paradigm.

\textbf{Reservoir} is a powerful baseline for balanced data streams~\cite{chaudhry2019continual}, with only minimal computational cost by keeping count $n$ of how many samples have been observed. This count is then used relative to the buffer size $M$ to define the probability $M/n$ to store the new sample.
As shown in the imbalanced data stream experiments, Reservoir is not fit for more real-world scenarios with typically varying frequency of occurrence per class. Improving this simple experience replay has led to research focusing on more complex strategies, discussed in the following.

\textbf{MIR}~\cite{aljundi2019online} replaces the random retrieval from the buffer in Reservoir with a loss-based approach. They store a momentary update of the network optimized for the new incoming batch and calculate the change in loss for a random subset of replay memories $\Tilde{B}$, which is larger than the batch size (ideally five times the batch size for their experiments~\cite{aljundi2019online}). 
Besides a copy of the full model, this also requires calculating the loss twice in a sequential manner for the full subset $\Tilde{B}$ and an extra temporary model update using only the new batch $B_n$, both significantly increasing processing time for the learner.

\textbf{GSS}~\cite{aljundi2019gradient} resides with Reservoir to use random retrieval of the buffer, but proposes a gradient-based population strategy.
They introduce two variants, in which the first solves an Integer Quadratic Problem (IQP) with polynomial complexity w.r.t. the replay memory. As this is not scalable, they also propose a stochastic GSS-greedy variant.
This more efficient GSS-greedy approach requires an additional forward pass, loss calculation, and backwards pass to obtain the gradients for the full considered subset $\Tilde{B}$ in the memory. 
Additionally, it uses similarities of the gradients for stochastic sample selection in the replay memory $\mathcal{M}_r$, straining memory requirements as batch $B_n$ requires for each sample $|\Tilde{B}| + 1$ gradients to be accessed simultaneously to calculate $|\Tilde{B}|$ cosine similarities in the high-dimensional gradient-space. 


\textbf{CoPE (ours)} resembles Reservoir's memory population by keeping count of the samples per class-specific replay memory subset. 
The PPP-loss requires calculation of a similarity matrix with all the $d$-dimensional representations in the batch $B$. Using a normalized cosine similarity, this implies efficient matrix multiplication with the low-dimensional vectors.
This is in high contrast to GSS, which calculates cosine similarity in the full high-dimensional gradient space for additional samples that are not present in current batch $B$, and therefore requires additional costly forward and backward passes. 
Furthermore, in our prototypical approach the prototype momentum updates also rely solely on samples that are in the current batch $B$, hence requiring only minimal additional computation.
Comparing to both MIR and GSS, we don't require storing model copies or additional gradients, but merely store low-dimensional prototypes for each class, saving a significant amount of required storage space.
For example, a Resnet18 model requires $11.7$ million parameters to enable model copies or gradients, whereas our method even for $1000$-way classification with $d=1024$ would require only $9\%$ of the model capacity in memory for the prototypes.

\section{Extended ablation study}
\label{apdx:ablation}

\subsection{Ablation prototype momentum}
In all experiments, a high momentum is employed to update prototypes with the latent mean of the batch.
Table~\ref{tab:prototype} illustrates the influence of higher momentum ($\ge 0.9$). Compared to low momentum of $0.1$, Split-MNIST only gains a small margin of $0.45\%$, whereas Split-CIFAR10 and Split-CIFAR100 significantly improve with at least $3.0\%$ and $4.2\%$ respectively.
Using momentum prevents the prototype to rely solely on the current batch instances, and higher momentum values attain a more gradual change of the prototypes by stabilizing its trajectory in the ever-evolving latent space.

\begin{table}[!hbtp]
\centering
\caption{Ablation study changing momentum strength for prototype updates, reported in average accuracy~($\%$) over 5 runs. Higher momentum values ($\geq 0.9$) obtain better performance, especially for the CIFAR sequences, compared to low momentum ($0.1$).  }
\label{tab:prototype}
\begin{tabular}{@{}lllll@{}}
\toprule
         & \multicolumn{4}{c}{\textbf{Prototype Momentum}}                                                         \\ \midrule
         & \multicolumn{1}{c}{0.1} & \multicolumn{1}{c}{0.9} & \multicolumn{1}{c}{0.95} & \multicolumn{1}{c}{0.99} \\
Split-MNIST    & $93.49 \pm 0.70$        & $94.11 \pm 0.34$        & $93.96 \pm 0.30$         & $93.94 \pm 0.20$         \\
Split-CIFAR10  & $44.48 \pm 3.19$        & $48.02 \pm 2.49$        & $47.98 \pm 3.14$         & $48.92 \pm 1.32$         \\
Split-CIFAR100 & $15.79 \pm 1.16$        & $21.62 \pm 0.69$        & $21.56 \pm 0.58$         & $20.01 \pm 1.81$         \\ \bottomrule
\end{tabular}
\end{table}

\subsection{Ablation inter and intra-class variance terms PPP-loss}
In this section, the importance is scrutinized of the two loss components to enhance inter and intra-class variance in the PPP-loss. Table~\ref{tab:posneg} compares using only positive pairs from the batch in the attractor ($\mathcal{L}_{pos}$) or only negative pairs in the repellor ($\mathcal{L}_{neg}$) to the full-fledged PPP-loss ($\mathcal{L}$).
The attractor term shows competitive performance to the full PPP-loss for Split-MNIST, but deteriorates as the data streams become harder for the CIFAR setups. The repellor term is on par with the full PPP-loss for Split-MNIST and Split-CIFAR10, but collapses for Split-CIFAR100. The latter is challenging due to the high number of classes with only a batch size of 10, which impedes having pseudo-prototypes of all classes in the same batch. The PPP-loss incorporates both reduction of intra-class variance with the attractor term and increases inter-class variance with the repellor term, attaining state-of-the-art performance.

Besides isolating the attractor and repellor terms of the PPP-loss in the ablation study, we further investigate the weighing of the two terms during the lifetime of the learner in Figure~\ref{fig:lossweight}.
We average results over 5 runs for balanced Split-MNIST, finding the repellor to dominate. This trend is to be expected as the repellor term in \Eqref{eq:final_loss} has per instance a summation over all other class instances.
The attractor term has minimal influence especially for data presented for the first task. This indicates the samples in the binary latent space (having observed only two classes) majorly repelling rather than attracting samples.
The embedding network is still learning the initial features, and overlap in the two latent class distributions summed over the other class samples results in a prevailing repellor term.

\begin{table}[!hbtp]
\centering
\caption{Ablation using solely the attractor ($\mathcal{L}_{pos}$) or repellor ($\mathcal{L}_{neg}$) compared to using both terms in the PPP-loss ($\mathcal{L}$).}
\label{tab:posneg}
\begin{tabular}{@{}lccc@{}}
\toprule
 & \multicolumn{3}{c}{\textbf{PPP-loss}}                  \\ \midrule
                       & $\mathcal{L}$    & $\mathcal{L}_{pos}$   & $\mathcal{L}_{neg}$                 \\
Split-MNIST            & $\bf 93.94 \pm 0.20$  & $93.25 \pm 0.22$ & $\bf 93.84 \pm 0.48$                  \\
Split-CIFAR10          & $\bf 48.92 \pm 1.32$  & $30.96 \pm 3.58$ & $\bf 49.30 \pm 3.57$                  \\
Split-CIFAR100         & $\bf 21.62 \pm 0.69$  & $15.85 \pm 0.34$ & $9.43 \pm 0.94$                   \\ \bottomrule
\end{tabular}
\end{table}



\begin{figure}[!hbtp]
  \centering
  \includegraphics[clip,trim={0cm 0cm 0cm 0.2cm},width=0.85\linewidth]{img/ICLR/LOSS__2020-10-01_14:51.pdf}
    \caption{\label{fig:lossweight}
       Weighing (\%) between the positive loss term $\mathcal{L}_{pos}$ compared to the full PPP-loss $\mathcal{L}$, averaged over 5 runs of balanced Split-MNIST with standard deviation in blue. 
    }
\end{figure}

\subsection{Pseudo-prototype ablation visualization}
In the main paper we find in an ablation study that using pseudo-prototypes $\hat{\bf p}$ as proxy for the class-mean has significant improvements for the PPP-loss. Additionally, Figure~\ref{fig:ppabl} shows this in a 2-dimensional t-SNE space for the first seed of the balanced Split-MNIST experiment.
Including the pseudo-prototypes (\emph{incl. $\hat{\bf p}$}) illustrates a striking degree of inter-class variance in Figure~\ref{fig:ppabl}a, whereas more interference occurs when excluding the pseudo-prototypes in Figure~\ref{fig:ppabl}b. This is reflected in the performance, as including prototypes results in  $94.52\%$ accuracy, whereas excluding them has only $90.86\%$ for the first seed.

\begin{figure}[!hbtp]
\centering

\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{img/test.pdf}
      \caption{PPP-loss $-$ \textit{incl. $\hat{\bf p}$}}

  \label{fig:sub1}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{img/test_ponly.pdf}
      \caption{PPP-loss $-$ \textit{excl. $\hat{\bf p}$}}
  \label{fig:sub2}
\end{subfigure}
\caption{Split-MNIST first seed t-SNE representation of the test data $S_{eval}$, including (a) and excluding (b) the pseudo-prototypes $\hat{\bf p}$ in the PPP-loss.
}
\label{fig:ppabl}
\end{figure}








\section{Additional experiments}
\label{apdx:extra_exps}
\subsection{Balanced data streams with low capacity}
\label{apdx:extra_exps:lowcap}
In these experiments we scrutinize performance of CoPE with less capacity in the memory and model, and with shorter data streams.
All methods are allowed multiple iterations (maximal 5) as in \cite{aljundi2019gradient}. Results are averaged over 5 seeds.
Similar to the setup of GSS~\cite{aljundi2019gradient}, we adopt two data sequences with truncated data per task:
\begin{itemize}
    \item \textbf{Split-MNIST-mini} is similar to the Split-MNIST data stream with 5 tasks, but each task is confined to 1k training samples. Evaluation considers the full test subset. The network is an MLP with two hidden layers of 100 units, with total memory size of $0.3$k exemplars. Latent dimensionality $d$ is selected $32$ from $[16,32,64]$.
\item \textbf{Split-CIFAR10-mini} is similar to the Split-CIFAR10 data stream with 5 tasks, but each task comprises 2k training samples, with a total subset of 10k samples out of the 50k available. The full test subset is used for evaluation. The network used is the same ResNet18 as in the main paper, with total memory size of $1$k exemplars. Latent dimensionality $d$ is selected $128$ from $[128, 256]$.
\end{itemize}

\paragraph{Analysis.}
Table~\ref{apdx:results_mini} shows the results for Split-MNIST-mini and Split-CIFAR10-mini, with GSS and DN-CPM results reported from their original works in a corresponding setup.
In Split-MNIST-mini our method approaches the iid-online baseline up to $1\%$, and outperforms its closest competitors GEM and MIR with at least $1.45\%$.
In Split-CIFAR10-mini CoPE saliently surpasses the iid-online baseline with $2.25\%$, hence outperforming online training over an iid datastream. Moreover, CoPE surpasses CN-DPM by $3\%$. Reservoir proves a strong baseline, with in this case the additional MIR loss-based retrieval decreasing performance. 
Similar to our findings in the main paper and \cite{aljundi2019online, aljundi2019gradient}, GEM encounters difficulties in a CIFAR10 based setup, for which we find the bias hyperparameter $\gamma \geq 0$ in the gradient projection to have insignificant influence.
These results confirm CoPE outperforming both GSS and CN-DPM in this low capacity setting established in their original work.


\begin{table}[!hbtp]
\centering
\caption{Split-MNIST-mini and  Split-CIFAR10-mini results, with respectively only $1$k and $2$k samples per task. GSS and DN-CPM results reported from original work in these setups.}
\label{apdx:results_mini}
\begin{tabular}{@{}lcc@{}}
\toprule
            & \textbf{Split-MNIST-mini} & \textbf{Split-CIFAR10-mini}    \\ \midrule
iid-offline & $94.58 \pm 0.17$     & $67.41 \pm 1.37$          \\
iid-online  & $87.57 \pm 3.54$     & $42.50 \pm 2.15$          \\ \midrule
finetune    & $21.74 \pm 3.38$     & $16.65 \pm 0.24$          \\
GEM         & $85.09 \pm 0.52$     & $22.31 \pm 1.37$          \\
iCaRL       & $83.23 \pm 0.92$     & $26.54 \pm 2.73$          \\ 
DN-CPM \cite{lee2020neural}      & $-$                 & $41.78$                   \\
reservoir   & $82.73 \pm 2.39$     & $38.21 \pm 3.39$          \\
MIR         & $84.40 \pm 0.91$     & $37.20 \pm 2.74$          \\
GSS~\cite{aljundi2019gradient}         & $82.60 \pm 2.90$     & $33.56 \pm 1.70$          \\
CoPE        & $ \bf 86.54 \pm 1.41$     & \textbf{$\bf 44.75 \pm 2.68$} \\ \bottomrule
\end{tabular}%
\end{table}


\subsection{Buffer size analysis: Split-CIFAR100}
The results for Split-CIFAR10 and Split-MNIST are reported in the main paper, whereas Split-CIFAR100 results are added here in Figure~\ref{fig:CIFAR100_buffer} due to lack of space. We observe the same trend, where CoPE prevails over other replay methods by high margin from low to high-capacity regimes. The performance of the learner in CoPE scales with the size of $\mathcal{M}_r$.

\begin{figure}[!hbtp]
  \centering
  \includegraphics[clip,trim={0cm 0cm 0cm 0.2cm},width=0.7\linewidth]{img/ICLR/BUFFER_COMP_cifar100__2020-09-25_09:18.pdf}
    \caption{\label{fig:CIFAR100_buffer}
       Accuracies over buffer sizes $|\mathcal{M}|$ for balanced Split-CIFAR100 sequence.
    }
\end{figure}



\subsection{Imbalanced Benchmark Results}
The graphs in the main paper visualize the numbers in Table~\ref{tab:unbal-exps}, which we fully report here as a reference for future work. Each $S(T_i)$ data stream performance is averaged  over five different initial seeds. The '\emph{Avg.}' results average over all mean performances of the dataset variants $S(T_i)$.



\begin{table*}[t]
\centering
\begin{tabular}{@{}cclllll@{}}
\toprule
\multicolumn{1}{c}{\textbf{Dataset}} & \multicolumn{1}{c}{\textbf{\textbf{\begin{tabular}[c]{@{}c@{}}Imbalanced\\ Sequence\end{tabular}}}} & \multicolumn{1}{c}{\textbf{CoPE}}& \multicolumn{1}{c}{\textbf{CoPE-CE}} & \multicolumn{1}{c}{\textbf{GSS}} & \multicolumn{1}{c}{\textbf{MIR}} & \multicolumn{1}{c}{\textbf{Reservoir}} \\ \midrule
\textbf{Split-MNIST}                & $S(T_1)$ & $83.4 \pm 2.0$ & $81.8 \pm 1.2$ & $75.9 \pm 3.2$ & $64.8 \pm 5.1$ & $64.2 \pm 2.3$ \\
                                    & $S(T_2)$ & $84.5 \pm 1.6$ & $80.1 \pm 1.9$ & $78.5 \pm 2.7$ & $67.4 \pm 3.2$ & $65.5 \pm 4.6$ \\
                                    & $S(T_3)$ & $85.1 \pm 0.6$ & $79.6 \pm 2.0$ & $81.5 \pm 2.3$ & $72.4 \pm 3.0$ & $72.1 \pm 4.0$ \\
                                    & $S(T_4)$ & $84.8 \pm 1.0$ & $80.0 \pm 3.1$ & $79.5 \pm 0.6$ & $72.6 \pm 3.1$ & $73.6 \pm 2.4$ \\
                                    & $S(T_5)$ & $84.0 \pm 1.3$ & $80.7 \pm 1.8$ & $79.1 \pm 0.7$ & $77.2 \pm 3.4$ & $73.2 \pm 4.0$ \\ \midrule
                                    & Avg.     & $\bf 84.4 \pm 0.7$ & $80.4 \pm 0.9$ & $78.9 \pm 2.0$ & $70.9 \pm 4.9$ & $69.7 \pm 4.5$ \\  \midrule\midrule\addlinespace
\textbf{Split-CIFAR10} & $S(T_1)$ & $39.0 \pm 1.3$ & $36.4 \pm 3.0$ & $32.3 \pm 3.0$ & $32.6 \pm 3.6$ & $35.5 \pm 3.4$ \\
                                    & $S(T_2)$ & $35.3 \pm 2.6$ & $34.1 \pm 2.8$ & $28.3 \pm 0.4$ & $27.2 \pm 1.8$ & $29.3 \pm 2.8$ \\
                                    & $S(T_3)$ & $36.2 \pm 2.5$ & $34.6 \pm 2.5$ & $29.5 \pm 1.5$ & $29.6 \pm 2.1$ & $31.4 \pm 2.1$ \\
                                    & $S(T_4)$ & $39.1 \pm 2.4$ & $33.5 \pm 4.2$ & $34.6 \pm 1.3$ & $31.0 \pm 2.3$ & $32.1 \pm 0.6$ \\
                                    & $S(T_5)$ & $37.3 \pm 3.3$ & $33.9 \pm 2.9$ & $28.3 \pm 2.4$ & $27.6 \pm 2.7$ & $28.8 \pm 1.9$ \\ \midrule
                                    & Avg.     & $\bf 37.4 \pm 1.7$ & $34.5 \pm 1.1$ & $30.6 \pm 2.8$ & $29.6 \pm 2.3$ & $31.4 \pm 2.7$ \\ \midrule\midrule\addlinespace
\textbf{Split-CIFAR100} & $S(T_1)$                                                               & $18.2 \pm 0.6$          & $11.7 \pm 0.6$ & $10.2 \pm 0.8$ & $18.4 \pm 0.9$ & $11.1 \pm 0.6$ \\
               & $S(T_5)$                                                               & $18.5 \pm 1.3$          & $12.6 \pm 1.2$ & $10.7 \pm 0.5$ & $17.6 \pm 0.9$ & $11.5 \pm 1.4$ \\
               & $S(T_{10})$                                                              & $19.2 \pm 0.9$          & $11.1 \pm 0.7$ & $11.1 \pm 0.3$ & $17.8 \pm 0.7$ & $11.9 \pm 0.7$ \\
               & $S(T_{15})$                                                              & $18.7 \pm 0.6$          & $11.2 \pm 0.8$ & $11.1 \pm 0.9$ & $17.8 \pm 0.9$ & $12.1 \pm 0.8$ \\
               & $S(T_{20})$                                                              & $18.5 \pm 1.5$          & $12.8 \pm 1.3$ & $11.1 \pm 0.4$ & $17.6 \pm 0.4$ & $12.5 \pm 1.1$ \\ \midrule
               & Avg.                                                                   & \textbf{$\bf 18.6 \pm 0.4$} & $11.9 \pm 0.8$ & $10.8 \pm 0.4$ & $17.8 \pm 0.3$ & $11.8 \pm 0.5$ \\ \midrule\bottomrule
\end{tabular}
\caption{\label{tab:unbal-exps}Numeric results for imbalanced Split-MNIST, Split-CIFAR10 and Split-CIFAR100 sequences.
}
\end{table*}



